Boosting Vision-Language Models with Transduction

Transduction is a powerful paradigm that leverages the structure of unlabeled data to boost predictive accuracy. We present TransCLIP, a novel and computationally efficient transductive approach designed for Vision-Language Models (VLMs). TransCLIP is applicable as a plug-and-play module on top of popular inductive zero- and few-shot models, consistently improving their performances. Our new objective function can be viewed as a regularized maximum-likelihood estimation, constrained by a KL divergence penalty that integrates the text-encoder knowledge and guides the transductive learning process. We further derive an iterative Block Majorize-Minimize (BMM) procedure for optimizing our objective, with guaranteed convergence and decoupled sample-assignment updates, yielding computationally efficient transduction for large-scale datasets. We report comprehensive evaluations, comparisons, and ablation studies that demonstrate: (i) Transduction can greatly enhance the generalization capabilities of inductive pretrained zero- and few-shot VLMs; (ii) TransCLIP substantially outperforms standard transductive few-shot learning methods relying solely on vision features, notably due to the KL-based language constraint.

==> Styles/figures/ablation_sample_size.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Styles/figures/plot_transclip_sample_size.pdf}
    \caption{Increasing query set size (50 random seeds).}
    \label{fig:ablation_query_size}
\end{figure}

==> Styles/tables/table_ablation_old.tex <==
% Define a slightly darker green 
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkred}{rgb}{0.8,0,0}
\begin{table}
\caption{Ablation study of several components of TransCLIP on the ImageNet dataset in the zero-shot setting.} \label{tab:ablation}

%\sisetup{table-format=-1.2}   % 2 decimals, leave 
\centering
\resizebox{0.7\linewidth}{!}{
   \begin{tabular}{lccccc}
\toprule
\multicolumn{1}{l}{\makecell{\bf Summary}}
& \multicolumn{1}{c}{\makecell{\bf (Update $\boldsymbol{\mu}$)}}
&\multicolumn{1}{c}{\makecell{\bf (Update $\boldsymbol{\Sigma}$)}}
& \multicolumn{1}{c}{\makecell{\bf (Text regularization $\hat{{\mathbf y}}$)}}
&\multicolumn{1}{c}{\makecell{\bf (Laplacian term $w$)}} 
&\multicolumn{1}{c}{\makecell{\bf Top-1 Accuracy}}
\\ 
\midrule
 Initialization & \textcolor{darkred}{\xmark} & \textcolor{darkred}{\xmark}  & \textcolor{darkred}{\xmark}  & \textcolor{darkred}{\xmark}  &  60.73  \\

$\boldsymbol{\mu}$ & \textcolor{darkgreen}{\cmark} & \textcolor{darkred}{\xmark}  & \textcolor{darkred}{\xmark}  & \textcolor{darkred}{\xmark} & 0.1  \\

$\boldsymbol{\mu}, \boldsymbol{\Sigma}$ & \textcolor{darkgreen}{\cmark} & \textcolor{darkgreen}{\cmark} & \textcolor{darkred}{\xmark}  & \textcolor{darkred}{\xmark}  & 0.1  \\
 $\boldsymbol{\mu}, \hat{{\mathbf y}}$ & \textcolor{darkgreen}{\cmark} & \textcolor{darkred}{\xmark}  & \textcolor{darkgreen}{\cmark}  & \textcolor{darkred}{\xmark}  & 66.73  \\

$\boldsymbol{\mu}, \hat{{\mathbf y}}, w$& \textcolor{darkgreen}{\cmark} & \textcolor{darkred}{\xmark} & \textcolor{darkgreen}{\cmark}   & \textcolor{darkgreen}{\cmark}  &  67.39 \\
$\boldsymbol{\mu}, \boldsymbol{\Sigma}, \hat{{\mathbf y}}$ & \textcolor{darkgreen}{\cmark} & \textcolor{darkgreen}{\cmark}  & \textcolor{darkgreen}{\cmark} & \textcolor{darkred}{\xmark}  &  69.93  \\

\rowcolor{LightGray} $\boldsymbol{\mu}, \boldsymbol{\Sigma}, \hat{{\mathbf y}}, w$ & \textcolor{darkgreen}{\cmark} & \textcolor{darkgreen}{\cmark} & \textcolor{darkgreen}{\cmark} &  \textcolor{darkgreen}{\cmark}  &  \textbf{70.29}  \\
      \bottomrule
   \end{tabular}}
\end{table}
